M3PT: A Transformer for Multimodal, Multi-Party Social Signal Prediction with Person-aware Blockwise Attention

Understanding social signals in multi-party conversations is important for human-robot interaction and artificial social intelligence. Social signals include body pose, head pose, speech, and context-specific activities like acquiring and taking bites of food when dining. Past work in multi-party interaction tends to build task-specific models for predicting social signals. In this work, we address the challenge of predicting multimodal social signals in multi-party settings in a single model. We introduce M3PT, a causal transformer architecture with modality and temporal blockwise attention masking to simultaneously process multiple social cues across multiple participants and their temporal interactions. We train and evaluate M3PT on the Human-Human Commensality Dataset (HHCD), and demonstrate that using multiple modalities improves bite timing and speaking status prediction. Source code: https://github.com/AbrarAnwar/masked-social-signals/.

==> Tables/triplet_ablation1.tex <==
% \begin{table*}[!t]
%      \caption{\textbf{Does \method\ learn from longer temporal context?}. We maintain the segment size of each token to be 3 seconds, and modify the number of seconds. Functionally, this allows the transformer to make predictions with longer contexts. We find that as the total amount of time increases, there is  decrease in precision for speaking status (S), while an increase in precision for bite timing (B). This result indicates that more temporal context can improve performance.}
%     \label{tab:ablation_study}
%     \centering
%     \begin{tabular}{cccccccc}
%         \toprule
% \multirow{2}{*}{\shortstack{Total Time \\ in Context}} & \multirow{2}{*}{\shortstack{Number of \\ Segments}} & Task & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{Precision} & \textbf{Recall} & \textbf{nMCC} \\ 
% & & & & & & &\\
% \midrule
%         6s & 2 & S & 0.99{\scriptsize $\pm$ 0.00} & 0.99{\scriptsize $\pm$ 0.00} & 0.99{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.99{\scriptsize $\pm$ 0.00} \\ 
%         ~ & ~ & B & 0.96{\scriptsize $\pm$ 0.03} & 0.89{\scriptsize $\pm$ 0.09} & 0.82{\scriptsize $\pm$ 0.15} & 0.99{\scriptsize $\pm$ 0.00} & 0.94{\scriptsize $\pm$ 0.05} \\ \midrule
%         9s & 3 & S & 0.99{\scriptsize $\pm$ 0.00} & 0.99{\scriptsize $\pm$ 0.00} & 0.99{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.99{\scriptsize $\pm$ 0.00} \\ 
%         ~ & ~ & B & 0.98{\scriptsize $\pm$ 0.01} & 0.89{\scriptsize $\pm$ 0.09} & 0.82{\scriptsize $\pm$ 0.15} & 1.00{\scriptsize $\pm$ 0.00} & 0.94{\scriptsize $\pm$ 0.04} \\ \midrule
%         18s & 6 & S & 0.91{\scriptsize $\pm$ 0.00} & 0.85{\scriptsize $\pm$ 0.00} & 0.74{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.90{\scriptsize $\pm$ 0.00} \\ 
%         ~ & ~ & B & 0.97{\scriptsize $\pm$ 0.00} & 0.87{\scriptsize $\pm$ 0.00} & 0.78{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.93{\scriptsize $\pm$ 0.00} \\ \midrule
%         36s & 12 & S & 0.93{\scriptsize $\pm$ 0.00} & 0.88{\scriptsize $\pm$ 0.00} & 0.79{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.92{\scriptsize $\pm$ 0.00} \\ 
%         ~ & ~ & B & 0.99{\scriptsize $\pm$ 0.00} & 0.95{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.91{\scriptsize $\pm$ 0.00} & 0.97{\scriptsize $\pm$ 0.00} \\ 
%         \bottomrule
%     \end{tabular}
    
% \end{table*}


\begin{table}[!t]
     \caption{\textbf{Does \method\ learn from longer temporal context?}. We maintain the segment size of each token to be 3 seconds, and modify the number of seconds. Functionally, this allows the transformer to make predictions with longer contexts. We find that as the total amount of time increases, there is  decrease in precision for speaking status (S), while an increase in precision for bite timing (B). This result indicates that more temporal context can improve performance.}
    \label{tab:ablation_study}
    \centering
    \begin{tabular}{c@{}ccccc}
        \toprule
 & Task & \textbf{F1 Score} & \textbf{Precision} & \textbf{Recall} & \textbf{nMCC} \\ 
\midrule
        \multirow{2}{*}{2$\times$3s} & S & 0.99{\scriptsize $\pm$ 0.00} & 0.99{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.99{\scriptsize $\pm$ 0.00} \\ 
         & B & 0.89{\scriptsize $\pm$ 0.09} & 0.82{\scriptsize $\pm$ 0.15} & 0.99{\scriptsize $\pm$ 0.00} & 0.94{\scriptsize $\pm$ 0.05} \\ \midrule
        \multirow{2}{*}{3$\times$3s} & S & 0.99{\scriptsize $\pm$ 0.00} & 0.99{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.99{\scriptsize $\pm$ 0.00} \\ 
        & B & 0.89{\scriptsize $\pm$ 0.09} & 0.82{\scriptsize $\pm$ 0.15} & 1.00{\scriptsize $\pm$ 0.00} & 0.94{\scriptsize $\pm$ 0.04} \\ \midrule
        \multirow{2}{*}{6$\times$3s} & S & 0.85{\scriptsize $\pm$ 0.00} & 0.74{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.90{\scriptsize $\pm$ 0.00} \\ 
        & B & 0.87{\scriptsize $\pm$ 0.00} & 0.78{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.93{\scriptsize $\pm$ 0.00} \\ \midrule
         \multirow{2}{*}{12$\times$3s} & S & 0.88{\scriptsize $\pm$ 0.00} & 0.79{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.92{\scriptsize $\pm$ 0.00} \\ 
        & B & 0.95{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.91{\scriptsize $\pm$ 0.00} & 0.97{\scriptsize $\pm$ 0.00} \\ 
        \bottomrule
    \end{tabular}
    
\end{table}

==> Tables/triplet_ablation2.tex <==
% \begin{table*}[!t]
%      \caption{
%     \textbf{Impact of Segment Length on Performance.} We hold the total time to be at a constant 36 seconds, but modify the length of a segment and thus the number of segments. We find that longer segment lengths leads to a collapse in performance in both speaking status prediction (S) and bite timing prediction (B) tasks degrade in performance as the segment length increases.
%     }
%     \centering
%     \begin{tabular}{cccccccc}
%         \toprule
%         \multirow{2}{*}{\shortstack{Number of \\ Segments}}  & \multirow{2}{*}{\shortstack{Length of \\ Segment}} & Task & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{Precision} & \textbf{Recall} & \textbf{nMCC} \\ 
%         & & & & & & &\\
%         \midrule
%         2 & 18s & S & 0.75{\scriptsize $\pm$ 0.00} & 0.00{\scriptsize $\pm$ 0.00} & 0.00{\scriptsize $\pm$ 0.00} & 0.00{\scriptsize $\pm$ 0.00} & 0.50{\scriptsize $\pm$ 0.00} \\ 
%         ~ & ~ & B & 0.82{\scriptsize $\pm$ 0.13} & 0.09{\scriptsize $\pm$ 0.13} & 0.06{\scriptsize $\pm$ 0.09} & 0.17{\scriptsize $\pm$ 0.24} & 0.53{\scriptsize $\pm$ 0.01} \\ \midrule
%         4 & 9s & S & 0.69{\scriptsize $\pm$ 0.13} & 0.11{\scriptsize $\pm$ 0.15} & 0.08{\scriptsize $\pm$ 0.11} & 0.16{\scriptsize $\pm$ 0.23} & 0.51{\scriptsize $\pm$ 0.00} \\ 
%         ~ & ~ & B & 0.26{\scriptsize $\pm$ 0.06} & 0.41{\scriptsize $\pm$ 0.08} & 0.26{\scriptsize $\pm$ 0.06} & 1.00{\scriptsize $\pm$ 0.00} & 0.48{\scriptsize $\pm$ 0.00} \\ \midrule
%         6 & 6s & S & 0.52{\scriptsize $\pm$ 0.18} & 0.22{\scriptsize $\pm$ 0.16} & 0.15{\scriptsize $\pm$ 0.10} & 0.45{\scriptsize $\pm$ 0.32} & 0.50{\scriptsize $\pm$ 0.01} \\ 
%         ~ & ~ & B & 0.23{\scriptsize $\pm$ 0.03} & 0.32{\scriptsize $\pm$ 0.07} & 0.19{\scriptsize $\pm$ 0.05} & 1.00{\scriptsize $\pm$ 0.00} & 0.52{\scriptsize $\pm$ 0.03} \\ \midrule
%         12 & 3s & S & 0.93{\scriptsize $\pm$ 0.00} & 0.88{\scriptsize $\pm$ 0.00} & 0.79{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.92{\scriptsize $\pm$ 0.00} \\ 
%         ~ & ~ & B & 0.99{\scriptsize $\pm$ 0.00} & 0.95{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.91{\scriptsize $\pm$ 0.00} & 0.97{\scriptsize $\pm$ 0.00} \\ 
%         \bottomrule
%     \end{tabular}
%     % \caption{This table presents the results of an ablation study where the total time is kept constant, but different segmenting strategies are applied by varying the segment length (in seconds) and the number of segments.}
   
%     \label{tab:ablation_segmenting}
% \end{table*}


\begin{table}[!t]
     \caption{
    \textbf{Impact of Segment Length on Performance.} We hold the total time to be at a constant 36 seconds, but modify the length of a segment and thus the number of segments. We find that longer segment lengths leads to a collapse in performance in both speaking status prediction (S) and bite timing prediction (B) tasks degrade in performance as the segment length increases.
    }
    \centering
    \begin{tabular}{c@{}ccccc}
        \toprule
            & Task & \textbf{F1 Score} & \textbf{Precision} & \textbf{Recall} & \textbf{nMCC} \\ 
        \midrule
        \multirow{2}{*}{2$\times$18s} & S & 0.00{\scriptsize $\pm$ 0.00} & 0.00{\scriptsize $\pm$ 0.00} & 0.00{\scriptsize $\pm$ 0.00} & 0.50{\scriptsize $\pm$ 0.00} \\ 
         & B & 0.09{\scriptsize $\pm$ 0.13} & 0.06{\scriptsize $\pm$ 0.09} & 0.17{\scriptsize $\pm$ 0.24} & 0.53{\scriptsize $\pm$ 0.01} \\ \midrule
        \multirow{2}{*}{4$\times$9s} & S & 0.11{\scriptsize $\pm$ 0.15} & 0.08{\scriptsize $\pm$ 0.11} & 0.16{\scriptsize $\pm$ 0.23} & 0.51{\scriptsize $\pm$ 0.00} \\ 
        & B & 0.41{\scriptsize $\pm$ 0.08} & 0.26{\scriptsize $\pm$ 0.06} & 1.00{\scriptsize $\pm$ 0.00} & 0.48{\scriptsize $\pm$ 0.00} \\ \midrule
        \multirow{2}{*}{6$\times$6s} & S & 0.22{\scriptsize $\pm$ 0.16} & 0.15{\scriptsize $\pm$ 0.10} & 0.45{\scriptsize $\pm$ 0.32} & 0.50{\scriptsize $\pm$ 0.01} \\ 
        & B & 0.32{\scriptsize $\pm$ 0.07} & 0.19{\scriptsize $\pm$ 0.05} & 1.00{\scriptsize $\pm$ 0.00} & 0.52{\scriptsize $\pm$ 0.03} \\ \midrule
        \multirow{2}{*}{12$\times$3s} & S & 0.88{\scriptsize $\pm$ 0.00} & 0.79{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.92{\scriptsize $\pm$ 0.00} \\ 
        & B & 0.95{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.91{\scriptsize $\pm$ 0.00} & 0.97{\scriptsize $\pm$ 0.00} \\ 
        \bottomrule
    \end{tabular}
    % \caption{This table presents the results of an ablation study where the total time is kept constant, but different segmenting strategies are applied by varying the segment length (in seconds) and the number of segments.}
   
    \label{tab:ablation_segmenting}
\end{table}


==> Tables/triplet_biting.tex <==
% \begin{table*}[!t]
%     \caption{\textbf{Bite Timing Prediction}.
%     We show the performance of bite timing prediction across different sets of features. 
%     We find that using all available features leads to the best performance, with an accuracy of 0.99 and high precision (1.00) and nMCC (0.97). 
%     When individual features such as gaze, words, or speaker data are removed, performance declines significantly, particularly in F1 score and nMCC.
%     This indicates that these features are important in predicting bite timing. 
%     }
%     \centering
%     \begin{tabular}{lccccc}
%         \toprule
%         Features & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} & \textbf{nMCC} \\ 
%         \midrule
%         All Features & 0.99{\scriptsize $\pm$ 0.00} & 0.95{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.91{\scriptsize $\pm$ 0.00} & 0.97{\scriptsize $\pm$ 0.00} \\ \midrule
%         No Gaze & 0.88{\scriptsize $\pm$ 0.09} & 0.58{\scriptsize $\pm$ 0.30} & 0.52{\scriptsize $\pm$ 0.34} & 0.73{\scriptsize $\pm$ 0.26} & 0.77{\scriptsize $\pm$ 0.17} \\ 
%         No Headpose & 0.99{\scriptsize $\pm$ 0.00} & 0.95{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.91{\scriptsize $\pm$ 0.00} & 0.97{\scriptsize $\pm$ 0.00} \\ 
%         No Pose & 0.98{\scriptsize $\pm$ 0.01} & 0.89{\scriptsize $\pm$ 0.05} & 0.92{\scriptsize $\pm$ 0.10} & 0.87{\scriptsize $\pm$ 0.03} & 0.94{\scriptsize $\pm$ 0.03} \\ 
%         No Word & 0.96{\scriptsize $\pm$ 0.03} & 0.82{\scriptsize $\pm$ 0.15} & 0.83{\scriptsize $\pm$ 0.23} & 0.84{\scriptsize $\pm$ 0.05} & 0.90{\scriptsize $\pm$ 0.08} \\ 
%         No Speaker & 0.80{\scriptsize $\pm$ 0.16} & 0.59{\scriptsize $\pm$ 0.29} & 0.50{\scriptsize $\pm$ 0.34} & 0.84{\scriptsize $\pm$ 0.12} & 0.77{\scriptsize $\pm$ 0.16} \\ 
%         % No Bite & - & - & - & - & - \\ 
%         \midrule
%         % Speaker Only & - & - & - & - & - \\ 
%         Bite Only & 0.63{\scriptsize $\pm$ 0.09} & 0.25{\scriptsize $\pm$ 0.05} & 0.16{\scriptsize $\pm$ 0.03} & 0.64{\scriptsize $\pm$ 0.09} & 0.58{\scriptsize $\pm$ 0.03} \\ 
%         \bottomrule
%     \end{tabular}
    
%     \label{tab:bite_main}
% \end{table*}


\begin{table}[!t]
    \caption{\textbf{Bite Timing Prediction}.
    We show the performance of bite timing prediction across different sets of features. 
    We find that using all available features leads to the best performance, with an accuracy of 0.99 and high precision (1.00) and nMCC (0.97). 
    When individual features such as gaze, words, or speaker data are removed, performance declines significantly, particularly in F1 score and nMCC.
    This indicates that these features are important in predicting bite timing. 
    }
    \centering
    \begin{tabular}{lcccc}
        \toprule
        Features & \textbf{F1} & \textbf{Precision} & \textbf{Recall} & \textbf{nMCC} \\ 
        \midrule
        All Features & 0.95{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.91{\scriptsize $\pm$ 0.00} & 0.97{\scriptsize $\pm$ 0.00} \\ \midrule
        No Gaze & 0.58{\scriptsize $\pm$ 0.30} & 0.52{\scriptsize $\pm$ 0.34} & 0.73{\scriptsize $\pm$ 0.26} & 0.77{\scriptsize $\pm$ 0.17} \\ 
        No Headpose & 0.95{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.91{\scriptsize $\pm$ 0.00} & 0.97{\scriptsize $\pm$ 0.00} \\ 
        No Pose & 0.89{\scriptsize $\pm$ 0.05} & 0.92{\scriptsize $\pm$ 0.10} & 0.87{\scriptsize $\pm$ 0.03} & 0.94{\scriptsize $\pm$ 0.03} \\ 
        No Word & 0.82{\scriptsize $\pm$ 0.15} & 0.83{\scriptsize $\pm$ 0.23} & 0.84{\scriptsize $\pm$ 0.05} & 0.90{\scriptsize $\pm$ 0.08} \\ 
        No Speaker & 0.59{\scriptsize $\pm$ 0.29} & 0.50{\scriptsize $\pm$ 0.34} & 0.84{\scriptsize $\pm$ 0.12} & 0.77{\scriptsize $\pm$ 0.16} \\ 
        % No Bite & - & - & - & - & - \\ 
        \midrule
        % Speaker Only & - & - & - & - & - \\ 
        Bite Only & 0.25{\scriptsize $\pm$ 0.05} & 0.16{\scriptsize $\pm$ 0.03} & 0.64{\scriptsize $\pm$ 0.09} & 0.58{\scriptsize $\pm$ 0.03} \\ 
        \bottomrule
    \end{tabular}
    
    \label{tab:bite_main}
\end{table}


==> Tables/triplet_speaking.tex <==
% \begin{table*}[!t]
%     \caption{\textbf{Speaking Status Prediction}.
%     We find that the best results for speaking status prediction are achieved when all features are included.
%     Excluding bite timing causes a noticeable decline in performance, particularly in F1 score and nMCC, highlighting the importance of bite features for accurate prediction.
%     Other features, such as gaze and pose, also affect performance, but their removal leads to less pronounced prediction drops compared to bite timing prediction.
%     }
%     \centering
%     \begin{tabular}{lccccc}
%         \toprule
%         Features & \textbf{Accuracy} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} & \textbf{nMCC} \\ 
%         \midrule
%         All Features & 0.93{\scriptsize $\pm$ 0.00} & 0.88{\scriptsize $\pm$ 0.00} & 0.79{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.92{\scriptsize $\pm$ 0.00} \\ \midrule
%         No Gaze & 0.91{\scriptsize $\pm$ 0.02} & 0.85{\scriptsize $\pm$ 0.03} & 0.75{\scriptsize $\pm$ 0.05} & 1.00{\scriptsize $\pm$ 0.00} & 0.90{\scriptsize $\pm$ 0.02} \\ 
%         No Headpose & 0.93{\scriptsize $\pm$ 0.00} & 0.88{\scriptsize $\pm$ 0.00} & 0.79{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.92{\scriptsize $\pm$ 0.00} \\ 
%         No Pose & 0.91{\scriptsize $\pm$ 0.02} & 0.85{\scriptsize $\pm$ 0.03} & 0.75{\scriptsize $\pm$ 0.05} & 1.00{\scriptsize $\pm$ 0.00} & 0.90{\scriptsize $\pm$ 0.02} \\ 
%         No Word & 0.92{\scriptsize $\pm$ 0.01} & 0.86{\scriptsize $\pm$ 0.03} & 0.77{\scriptsize $\pm$ 0.03} & 0.97{\scriptsize $\pm$ 0.03} & 0.91{\scriptsize $\pm$ 0.02} \\ 
%         % Mask Speaker & - & - & - & - & - \\ 
%         No Bite & 0.87{\scriptsize $\pm$ 0.04} & 0.76{\scriptsize $\pm$ 0.11} & 0.70{\scriptsize $\pm$ 0.06} & 0.85{\scriptsize $\pm$ 0.19} & 0.84{\scriptsize $\pm$ 0.07} \\ \midrule
%         Speaker Only & 0.71{\scriptsize $\pm$ 0.02} & 0.53{\scriptsize $\pm$ 0.02} & 0.45{\scriptsize $\pm$ 0.04} & 0.66{\scriptsize $\pm$ 0.04} & 0.67{\scriptsize $\pm$ 0.01} \\ 
%         % Bite Only & - & - & - & - & - \\ 
%         \bottomrule
%     \end{tabular}
    
%     \label{tab:speaking_main}
% \end{table*}

\begin{table}[!t]
    \caption{\textbf{Speaking Status Prediction}.
    We find that the best results for speaking status prediction are achieved when all features are included.
    Excluding bite timing causes a noticeable decline in performance, particularly in F1 score and nMCC, highlighting the importance of bite features for accurate prediction.
    Other features, such as gaze and pose, also affect performance, but their removal leads to less pronounced prediction drops compared to bite timing prediction.
    }
    \centering
    \begin{tabular}{lcccc}
        \toprule
        Features & \textbf{F1} & \textbf{Precision} & \textbf{Recall} & \textbf{nMCC} \\ 
        \midrule
        All Features & 0.88{\scriptsize $\pm$ 0.00} & 0.79{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.92{\scriptsize $\pm$ 0.00} \\ \midrule
        No Gaze & 0.85{\scriptsize $\pm$ 0.03} & 0.75{\scriptsize $\pm$ 0.05} & 1.00{\scriptsize $\pm$ 0.00} & 0.90{\scriptsize $\pm$ 0.02} \\ 
        No Headpose & 0.88{\scriptsize $\pm$ 0.00} & 0.79{\scriptsize $\pm$ 0.00} & 1.00{\scriptsize $\pm$ 0.00} & 0.92{\scriptsize $\pm$ 0.00} \\ 
        No Pose & 0.85{\scriptsize $\pm$ 0.03} & 0.75{\scriptsize $\pm$ 0.05} & 1.00{\scriptsize $\pm$ 0.00} & 0.90{\scriptsize $\pm$ 0.02} \\ 
        No Word & 0.86{\scriptsize $\pm$ 0.03} & 0.77{\scriptsize $\pm$ 0.03} & 0.97{\scriptsize $\pm$ 0.03} & 0.91{\scriptsize $\pm$ 0.02} \\ 
        % Mask Speaker & - & - & - & - & - \\ 
        No Bite & 0.76{\scriptsize $\pm$ 0.11} & 0.70{\scriptsize $\pm$ 0.06} & 0.85{\scriptsize $\pm$ 0.19} & 0.84{\scriptsize $\pm$ 0.07} \\ \midrule
        Speaker Only & 0.53{\scriptsize $\pm$ 0.02} & 0.45{\scriptsize $\pm$ 0.04} & 0.66{\scriptsize $\pm$ 0.04} & 0.67{\scriptsize $\pm$ 0.01} \\ 
        % Bite Only & - & - & - & - & - \\ 
        \bottomrule
    \end{tabular}
    
    \label{tab:speaking_main}
\end{table}



==> figs/teaser.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{example-image-duck}
    \caption{THIS IS THE OVERVIEW FIGURE
    \textit{Left:} Previous methods for identifying object referents of language expressions in the SNARE~\cite{thomason_language_2021} benchmark reason about target and distractor objects independently and pool multi-view information before grounding.
    \textit{Right:} By contrast, {\model} jointly reasons over target and distractor objects and their views from different angles to identify the correct referent with higher accuracy than the previous state-of-the-art model.
    }
    \label{fig:overview}
\end{figure}


